Convolutional Phase Retrieval via Gradient Descent

We study the convolutional phase retrieval problem, of recovering an unknown signal $\mathbf x \in \mathbb C^n $ from $m$ measurements consisting of the magnitude of its cyclic convolution with a given kernel $\mathbf a \in \mathbb C^m $. This model is motivated by applications such as channel estimation, optics, and underwater acoustic communication, where the signal of interest is acted on by a given channel/filter, and phase information is difficult or impossible to acquire. We show that when $\mathbf a$ is random and the number of observations $m$ is sufficiently large, with high probability $\mathbf x$ can be efficiently recovered up to a global phase shift using a combination of spectral initialization and generalized gradient descent. The main challenge is coping with dependencies in the measurement operator. We overcome this challenge by using ideas from decoupling theory, suprema of chaos processes and the restricted isometry property of random circulant matrices, and recent analysis of alternating minimization methods.

==> sections/geometry.tex <==
\section{Analysis of the Geometry}
 
\subsection{Sketch}
Despite the special dependence structure within the sampling matrix $\mb A$, as long as the these two models follow the same random distribution, the same expectation will fall out and implies resembleness in the general geometry.
\begin{lemma}\label{lem:expect-func}
For the function $f(\mb z): \bb C^n \mapsto \bb R$ defined earlier, have
\begin{align}
\expect{f(\mb z)} &= \norm{\mb x}{}^4 + \norm{\mb z}{}^4 - \norm{\mb x}{}^2 \norm{\mb z}{}^2 - \abs{\mb x^* \mb z}^2,  \label{eqn:expect-f} \\
\nabla \expect{f(\mb z)} &= \begin{bmatrix}\nabla_{\mb z} \expect{f(\mb z)} \\
\nabla_{\ol{\mb z}} \expect{f(\mb z)}\end{bmatrix} 
= \begin{bmatrix}\paren{2\norm{\mb z}{}^2 \mb I - \norm{\mb x}{}^2 \mb I - \mb x \mb x^*} \mb z \\
\paren{2\norm{\mb z}{}^2\mb I  - \norm{\mb x}{}^2 \mb I - \mb x \mb x^*} \ol{\mb z} 
\end{bmatrix}, \label{eqn:expect-grad} \\
\nabla^2 \expect{f(\mb z)} &= \begin{bmatrix}
2 \mb z \mb z^* - \mb x \mb x^* + \paren{2\norm{\mb z}{}^2 - \norm{\mb x}{}^2} \mb I & 2\mb z \mb z^\top  \\
2 \ol{\mb z} \mb z^* & 2 \ol{\mb z} \mb z^\top - \ol{\mb x} \mb x^\top + \paren{2\norm{\mb z}{}^2 - \norm{\mb x}{}^2} \mb I
\end{bmatrix}. \label{eqn:expect-hess}
\end{align}
\end{lemma}




\begin{lemma} \label{lem:fourth_exp}
For $\mb a \sim \mc{CN}(m)$ and any fixed vector $\mb x\in \bb C^n$, it holds that 
\begin{align*}
\expect{\abs{\mb a^* \mb x}^2 \mb a \mb a^*} = \mb x\mb x^* + \norm{\mb x}{}^2 \mb I,  \quad \text{and} \quad \expect{\paren{\mb a^* \mb x}^2 \mb a \mb a^\top} = 2 \mb x\mb x^\top. 
\end{align*}
\end{lemma}


Inspired by previous work by ???, the next thing would be to show the randomness is not going to generate a big perturbation. The argument about global geometry was carries through via a cover of 3 regions, each has certain property and together implies optimality. To be specific, region 1 has negative curvature; region 2 has large gradient and can be further chopped based on different gradient direction and region 3 is strongly convex and contains the ground truth and its symmetric solution. 
\begin{align*}
\frac{1}{\norm{\mb x}{}^2}
\begin{bmatrix}
\mb x \e^{\im \phi(\mb z)} \\
\ol{\mb x} \e^{-\im \phi(\mb z)}
\end{bmatrix}^*   \nabla^2 f(\mb z) 
\begin{bmatrix}
\mb x \e^{\im \phi(\mb z)}\\
\ol{\mb x} \e^{-\im \phi(\mb z)}
\end{bmatrix} 
\;& \le \;  
- \frac{1}{100} \norm{\mb x}{}^2, &\forall\; &  \mb z \in \mc R_1, &\quad \text{(Negative Curvature)} \\
 \frac{ \mb z^* \nabla_{\mb z} f(\mb z)}{\norm{\mb z}{}} \;&\ge \; \frac{1}{1000} \norm{\mb x}{}^2 \norm{\mb z}{},  & \forall\; & \mb z \in \mc R_2^{\mb z}, &\quad \text{(Large Gradient)} \\
 \frac{ \Re\paren{\mb h(\mb z)^* \nabla_{\mb z} f(\mb z)}}{ \norm{\mb h(\mb z)}{} } \;&\ge\; \frac{1}{1000} \norm{\mb x}{}^2 \norm{\mb z}{},  &\forall\; & \mb z \in \mc R_2^{\mb h}, &\quad \text{(Large Gradient)}\\
\begin{bmatrix}
\mb g(\mb z) \\
\ol{\mb g(\mb z)}
\end{bmatrix}^* 
\nabla^2 f(\mb z) 
\begin{bmatrix}
\mb g(\mb z) \\
\ol{\mb g(\mb z)}
\end{bmatrix} 
\;&\ge\; \frac{1}{4} \norm{\mb x}{}^2, &\forall\; &  \mb z \in \mc R_3, &\quad \text{(Restricted Strong Convexity)}
\end{align*}
and those regions cover the whole space $\mc R_1 \cup \mc R_2^{\mb z} \cup \mc R_2^{\mb h} \cup \mc R_3 = \Cp^n  $.


\begin{proposition}[Negative Curvature for $\mc R_1$]
 \label{prop:nega-curv}
When $m \ge Cn\log n$, it holds with probability at least $1 - c_a\exp\paren{-c_bm/\log m} - c_c m^{-1}$ that 
\begin{align*}
\frac{1}{\norm{\mb x}{}^2}
\begin{bmatrix}
\mb x \e^{\im \phi(\mb z)} \\
\ol{\mb x} \e^{-\im \phi(\mb z)}
\end{bmatrix}^*   \nabla^2 f(\mb z) 
\begin{bmatrix}
\mb x \e^{\im \phi(\mb z)}\\
\ol{\mb x} \e^{-\im \phi(\mb z)}
\end{bmatrix} 
\le 
- \frac{1}{100} \norm{\mb x}{}^2
\end{align*}
for all $\mb z \in \mc R_1\doteq\set{\mb z: 8\abs{\mb x^* \mb z}^2 + \frac{401}{100}\norm{\mb x}{}^2 \norm{\mb z}{}^2 \le \frac{398}{100} \norm{\mb x}{}^4 }$. Here $C$, and $c_a$ to $c_c$ are positive absolute constants. 
\end{proposition}
\begin{proof} For fixed $\mb x$
\begin{eqnarray}
\norm{\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\mb a_k\mb a_k^*- \paren{ \mb x \mb x^* + \norm{\mb x}{}^2 \mb I } }{}&\le&\delta\norm{\mb x}{2}^2\\
\norm{\frac{1}{m}\sum_{k=1}^m\paren{\mb a_k^*\mb x}^2\mb a_k\mb a_k^T- \mb x \mb x^T}{}&\le&\delta\norm{\mb x}{2}^2\\
\frac1m\sum_{k=1}^m\abs{\mb a_k^*\mb x}^4&\ge&\frac{399}{200}\|\mb x\|^4
\end{eqnarray}

\end{proof}


\begin{proposition}[Large Gradient for $\mc R_2^{\mb z}$]
\label{prop:grad-region-z}
When $m \ge Cn\log n$, it holds with probability at least $1 - c_a\exp(-c_b m/\log m) - c_c m^{-1}$ that 
\begin{align*}
\frac{\mb z^* \nabla_{\mb z} f(\mb z)}{\norm{\mb z}{}} \geq \frac{1}{1000} \norm{\mb x}{}^2 \norm{\mb z}{} 
\end{align*}
for all $\mb z \in \mc R_2^{\mb z}\doteq\set{\mb z: \Re\paren{\innerprod{\mb z}{\nabla_{\mb z} \expect{f}} } \ge \frac{1}{100} \norm{\mb z}{}^4 + \frac{1}{500} \norm{\mb x}{}^2 \norm{\mb z}{}^2 }$. Here $C$ and $c_a$ to $c_c$ are positive absolute constants. 
\end{proposition}
\begin{proof}For fixed $\mb x$ and all $\mb z$
\begin{eqnarray}
\norm{\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\mb a_k\mb a_k^*- \paren{ \mb x \mb x^* + \norm{\mb x}{}^2 \mb I } }{}&\le&\delta\norm{\mb x}{2}^2\\
\frac1m\sum_{k=1}^m\abs{\mb a_k^*\mb z}^4&\ge&\frac{199}{100}\|\mb z\|^4
\end{eqnarray}
\end{proof}

\begin{proposition}[Large Gradient for $\mc R_2^{\mb h}$]
\label{prop:grad-region-zx}
When $m \ge C n \log^3n$, it holds with probability at least $1 - c_a\exp(-c_b m/\log^2 m) - c_c m^{-1}$ that 
\begin{align*}
\Re\paren{\mb h(\mb z)^* \nabla_{\mb z} f(\mb z)} \geq  \frac{1}{1000} \norm{\mb x}{}^2 \norm{\mb z}{}\norm{\mb h(\mb z)}{}
\end{align*}
for all $\mb z \in \mc R_2^{\mb h}\doteq\left\{\mb z: \Re\paren{\innerprod{\mb h(\mb z) }{\nabla_{\mb z}\expect{f}}} \geq \frac{1}{250}\norm{\mb x}{}^2 \norm{\mb z}{} \norm{\mb h(\mb z)}{},\frac{11}{20} \norm{\mb x}{} \le \norm{\mb z}{} \le \norm{\mb x}{}, \mathrm{dist}(\mb z, \mc X) \ge \frac{\norm{\mb x}{}}{3} \right\}$. Here, $c_a$ to $c_c$ and $C$ are positive absolute constants. 
\end{proposition}
\begin{proof}Let $\mb h(\mb z)=\mb z-\mb xe^{i\phi(\mb z)}$, then
\[(\mb z - \mb x \e^{\im \phi} )^* \nabla_{\mb z} f(\mb z)
 = \frac{1}{m}\sum_{k=1}^m \abs{\mb a_k^* \mb z}^2 (\mb z - \mb x \e^{\im \phi} )^* \mb a_k \mb a_k^* \mb z - \frac{1}{m}\sum_{k=1}^m \abs{\mb a_k^* \mb x}^2 (\mb z - \mb x \e^{\im \phi} )^* \mb a_k \mb a_k^* \mb z.\]


\end{proof}


\begin{proposition}[Strong Convexity for $\mc R_3$]
\label{prop:str_cvx}
When $m \ge Cn\log n$ for a sufficiently large constant $C$, it holds with probability at least $1 - c_a m^{-1} - c_b\exp(-c_cm/\log m)$ that 
\begin{align*}
\begin{bmatrix}
\mb g(\mb z) \\
\ol{\mb g(\mb z)}
\end{bmatrix}^* 
\nabla^2 f(\mb z) 
\begin{bmatrix}
\mb g(\mb z) \\
\ol{\mb g(\mb z)}
\end{bmatrix} 
\ge \frac{1}{4} \norm{\mb x}{}^2 
\end{align*}
for all $\mb z \in \mc R_3\doteq\set{\mb z: \mathrm{dist}(\mb z, \mc X) \le \frac{1}{\sqrt{7}}\norm{\mb x}{}}$ and for all 
\begin{align*}
\mb g(\mb z) \doteq 
\begin{cases}
\paren{\mb z - \mb x \e^{\im \phi(\mb z)}}/\norm{\mb z - \mb x \e^{\im \phi(\mb z)}}{}  & \text{if}\; \mathrm{dist}(\mb z, \mc X) \neq 0, \\
\mb h \in \mc S \doteq \set{\mb h: \Im(\mb h^* \mb z) = 0, \norm{\mb h}{} = 1}   & \text{if}\; \mb z \in \mc X. 
\end{cases}
\end{align*}
Here $C$, $c_a$ to $c_c$ are positive absolute constants.  
\end{proposition}
\begin{proof}
\begin{eqnarray}
\norm{\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\mb a_k\mb a_k^*- \paren{ \mb x \mb x^* + \norm{\mb x}{}^2 \mb I } }{}&\le&\delta\norm{\mb x}{2}^2\\
\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\abs{\mb a_k^*\mb z}^2&\ge&(1-\delta)\paren{\norm{\mb x}2^2\norm{\mb z}2^2+\abs{\mb x^*\mb z}^2}
\end{eqnarray}
\end{proof}




\begin{itemize}
\item For any fixed $\mb x\in\Cp^n$, with probability at least $1-?$
\begin{eqnarray}
\norm{\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\mb a_k\mb a_k^*- \paren{ \mb x \mb x^* + \norm{\mb x}{}^2 \mb I } }{}&\le&\delta\norm{\mb x}{2}^2\\
\norm{\frac{1}{m}\sum_{k=1}^m\paren{\mb a_k^*\mb x}^2\mb a_k\mb a_k^T- \mb x \mb x^T}{}&\le&\delta\norm{\mb x}{2}^2
\end{eqnarray}


\item For Region $\mc R_3$, all $\mb x,\mb z\in\Cp^n$,with probability at least $1-?$
\begin{eqnarray}
\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\abs{\mb a_k^*\mb z}^2&\ge&(1-\delta)\paren{\norm{\mb x}2^2\norm{\mb z}2^2+\abs{\mb x^*\mb z}^2}\\
\frac{1}{m}\sum_{k=1}^m\Re\brac{(\mb a_k^*\mb x)(\mb z^*\mb a_k)}^2&\ge&(1-\delta)\paren{\frac12\norm{\mb x}2^2\norm{\mb z}2^2+\frac32\brac{\Re\mb x^*\mb w}^2-\frac12\brac{\mf I\mb x^*\mb z}^2}
\end{eqnarray}
\end{itemize}


\subsection{Two-sided bound I}

\begin{lemma}
When $m \geq n \log (n)$, we have
\begin{align}
\norm{\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\mb a_k\mb a_k^*- \paren{ \mb x \mb x^* + \norm{\mb x}{2}^2 \mb I } }{}\leq xx
\end{align}

with probability at least xx.
\end{lemma}

\begin{proof}
For simplicity, let
\begin{align}
\mb T(\mb a) \doteq \frac{1}{m} \sum_{k=1}^m \abs{\mb a_k^*\mb x}^2 \mb a_k \mb a_k^*
\end{align}
and its decoupled form can be expressed as
\begin{align}
\mb Q_{dec}(\mb a,\mb a') \doteq \frac{1}{m} \sum_{k=1}^m \abs{\mb a_k^*\mb x}^2 \mb a'_k (\mb a'_k)^*
\end{align}
Under assumption that $\mb a$ and $\mb a'$ are independent and follow complex Gaussian distribution $\mc{CN}(m)$, or $\mc{N}(0,\mb I_m/2)+i\mc{N}(0,\mb I_m/2)$, then
\begin{eqnarray}
\bar{\mb a}&=&\frac{\mb a+\mb a'}{2}\sim\mc{N}(0,\mb I_m/4)+i\mc{N}(0,\mb I_m/4)\\
\mb\delta&=&\frac{\mb a-\mb a'}{2}\sim\mc{N}(0,\mb I_m/4)+i\mc{N}(0,\mb I_m/4)
\end{eqnarray}
based on the conditioning argument for general decoupling 
\begin{eqnarray}
\mb Q(\bar{\mb a})&=&\expect{\mb Q_{dec}(\bar{\mb a}+\mb\delta,\bar{\mb a}-\mb\delta)}\\
&=&\mb T(\bar{\mb a})-\expect{\mb T(\bar{\mb a})}\\
&+&\frac1m\sum_{k=1}^m\brac{\frac12\bar{\mb a}_k\bar{\mb a}_k^*\|\mb x\|_2^2+\frac12\abs{\bar{\mb a}_k^*\mb x}^2\mb I-\mb x\mb x^*\bar{\mb a}_k\bar{\mb a}_k^*}\\
&+&\frac12\paren{\|\mb x\|_2^2\mb I_n+\mb x\mb x^*}
\end{eqnarray}
Hence
\begin{eqnarray}
\mb Q(\bar{\mb a})-\|\mb x\|_2^2\mb I_n&=&\mb T(\bar{\mb a})-\expect{\mb T(\bar{\mb a})}\\
&+&\frac1m\sum_{k=1}^m\frac12\bar{\mb a}_k\bar{\mb a}_k^*\|\mb x\|_2^2-\frac14\|\mb x\|_2^2\mb I_n\\
&+&\frac1m\sum_{k=1}^m\frac12\abs{\bar{\mb a}_k^*\mb x}^2\mb I-\frac14\|\mb x\|_2^2\mb I_n\\
&+&\frac12\mb x\mb x^*-\frac1m\sum_{k=1}^m\mb x\mb x^*\bar{\mb a}_k\bar{\mb a}_k^*
\end{eqnarray}
and the problem of bounding the operator norm of $\mb T(\bar{\mb a})-\expect{\mb T(\bar{\mb a})}$ can be reduced to bounding the  operator norm of $\Delta=\frac1m\sum_{k=1}^m\bar{\mb a}_k\bar{\mb a}_k^*-\frac12\mb I_n$.

\end{proof}

\begin{comment}
	\begin{lemma}\label{lem:cir-rip}
Let $\mb a_k\in\Cp^n$ be the $k$-th row of the sampling matrix $\mb A$ generated from standard complex Gaussian distribution $\mb a\sim\mc{CN}(m)$ and $m\ge c\delta^{-2}n\log^3{n}?$, then
\[\P\Brac{\norm{\frac1m\sum_{k=1}^m\mb a_k\mb a_k^*-\mb I_n}{}\le\delta}\ge1-\eta\]
\end{lemma}
\begin{proof}
Note that $\Delta=\frac1m\sum_{k=1}^m\mb a_k\mb a_k^*-\mb I_n$ is always a Hermitian matrix, which has real eigenvalues.\footnote{This special property is actually not that important.} 
\begin{eqnarray}
\norm{\frac1m\sum_{k=1}^m\mb a_k\mb a_k^*-\mb I_n}{}
&=&\sup_{\mb v\in\Cp^n,\norm{\mb v}2^2=1}\norm{\paren{\frac1m\sum_{k=1}^m\mb a_k\mb a_k^*-\mb I_n}\mb v}2\\
&=&\sup_{\mb v\in\Cp^n,\norm{\mb v}2^2=1}\abs{\mb v^*\paren{\frac1m\sum_{k=1}^m\mb a_k\mb a_k^*-\mb I_n}\mb v}\\
&=&\sup_{\mb v\in\Cp^n,\norm{\mb v}2^2=1}\abs{\frac1m\sum_{k=1}^m\abs{\mb a_k^*v}^2-\|\mb v\|^2}\\
&=&\sup_{\mb v\in\Cp^n,\norm{\mb v}2^2=1}\abs{\norm{\frac1{\sqrt{m}}\mb C_{\tilde{\mb v}}\mb a}2^2-\bb E_{\mb a}\norm{\frac1{\sqrt{m}}\mb C_{\tilde{\mb v}}\mb a}2^2}
\end{eqnarray}
Let's $\mc V = \set{\mb V\in\Cp^{m\times m}\mid\mb V=\frac1{\sqrt{m}}\mb C_{\tilde{\mb v}},\tilde{\mb v}=\imath\mb v,\mb v\in\Cp^n,\norm{\mb v}2^2=1}$, below quantities immediately follow
\[d_{F}(\mc V)=1\]
\[d_{2\to2}(\mc V)=\frac1{\sqrt{m}}\norm{\mc F\tilde{\mb v}}\infty=\frac1{\sqrt{m}}\norm{\mb v}1\le\sqrt{\frac{n}{m}}\norm{\mb v}2\]
\[\gamma_2(\mc V,\norm{\cdot}{2\to2})\le\sqrt{\frac{n}{m}}\log^{3/2}{n}\log^{1/2}{m}\]

To be more general, let $\mc U = \set{\mb U\in\Cp^{m\times m}\mid\mb U=\frac1{\sqrt{m}}\diag(\mb r)\mb C_{\tilde{\mb u}},\tilde{\mb u}=\imath\mb u,\mb u\in\Cp^n,\norm{\mb u}2^2=1}$. Here the other independent vector $\mb r=\mb C_{\mb v}\imath\mb x=\mb C_{\tilde{\mb x}}\mb v$, then $\norm{\mb r}{\infty}\le\sqrt{\log{m}}\norm{\mb x}2$ with some constant probability and $\norm{\frac1m\sum_{k=1}^m\abs{\mb v_k^*\mb x}^2\mb I-\|\mb x\|_2^2\mb I}2\le c$ with probability $1-m^{-c}$, hence
\[d_{F}(\mc U)=\frac{\norm{\mb r}2}{\sqrt{m}}\le c\]
\[d_{2\to2}(\mc U)=\sqrt{\frac{\log{m}}{m}}\norm{\mc F\tilde{\mb v}}\infty=\sqrt{\frac{\log{m}}{m}}\norm{\mb v}1\le\sqrt{\frac{n\log{m}}{m}}\norm{\mb v}2\]
\[\gamma_2(\mc U,\norm{\cdot}{2\to2})\le\sqrt{\frac{n}{m}}\log^{3/2}{n}\log^{3/2}{m}\]




Main arguments for the proof:
\begin{itemize}
\item Decoupling for 2nd order complex standard Gaussian random variables
\[\expect{\sup_{\mc V}\abs{\norm{\mb V\mb a}2^2-\bb E_{\mb a}\norm{\mb V\mb a}2^2}^p}\le C^p\expect{\sup_{\mc V}\abs{\innerprod{\mb V\mb a}{\mb V\mb a'}}^p}\]
\item Chaining
\[\norm{\sup_{\mc V}\abs{\innerprod{\mb V\mb a}{\mb V\mb a'}}}{p}\le\gamma_2(\mc V,\norm{\cdot}{2\to2})\norm{\sup_{\mc V}\norm{\mb V\mb a}2}{p}+\sup_{\mc V}\norm{\innerprod{\mb V\mb a}{\mb V\mb a'}}{p}\]
and for $L$-subgaussians
\[\norm{\sup_{\mc V}\norm{\mb V\mb a}2}{p}\le\gamma_2(\mc V,\norm{\cdot}{2\to2})+d_F(\mc V)+\sqrt{p}d_{2\to2}(\mc V)\]
\[\sup_{\mc V}\norm{\innerprod{\mb V\mb a}{\mb V\mb a'}}{p}\le\sqrt{p}d_{F}(\mc V)d_{2\to2}(\mc V)+pd^2_{2\to2}(\mc V)\]
\item By Markov's inequality, a random variable $v$ satisfies
\[\paren{\bb E\abs{v}^p}^{1/p}\le\alpha+\beta\sqrt{p}+\gamma p\quad\forall p\ge p_0\implies\prob{\abs{v}\le e\paren{\alpha+\beta\sqrt{u}+\gamma u}}\le e^{-u}\quad u\ge p_0\]
\end{itemize}

\end{proof}





\begin{lemma}
\[\frac1m\sum_{k=1}^m\abs{\mb a_k^*\mb x_0}^4\ge\delta\bb E\brac{\frac1m\sum_{k=1}^m\abs{\mb a_k^*\mb x_0}^4}\]
\end{lemma}
\begin{proof}
\begin{eqnarray}
\frac1m\sum_{k=1}^m\abs{\mb a_k^*\mb x_0}^4
&\ge&\frac1m\times m^{1/2-1/4}\sum_{k=1}^m\abs{\mb a_k^*\mb x_0}^2
\end{eqnarray}
\end{proof}

\end{comment}


\subsection{Two-sided bound II}
\begin{lemma}
When $m \geq n \log (n)$, we have
\begin{align}
\norm{\frac{1}{m}\sum_{k=1}^m\paren{\mb a_k^*\mb x}^2\mb a_k\mb a_k^T- \mb x \mb x^T}{}\le\delta\norm{\mb x}{2}^2
\end{align}
with probability at least xx.
\end{lemma}


\begin{proof}For simplicity, let
\begin{align}
\mb T(\mb a) \doteq \frac{1}{m} \sum_{k=1}^m \paren{\mb a_k^*\mb x}^2 \mb a_k \mb a_k^T
\end{align}
\begin{align}
\mb Q_{dec}(\mb a,\mb a') \doteq \frac{1}{m} \sum_{k=1}^m \paren{\mb a_k^*\mb x}^2 \mb a'_k (\mb a'_k)^T
\end{align}
Under assumption that $\mb a$ and $\mb a'$ are independent and follow complex Gaussian distribution $\mc{CN}(m)$, or $\mc{N}(0,\mb I_m/2)+i\mc{N}(0,\mb I_m/2)$, then
\begin{eqnarray}
\bar{\mb a}&=&\frac{\mb a+\mb a'}{2}\sim\mc{N}(0,\mb I_m/4)+i\mc{N}(0,\mb I_m/4)\\
\mb\delta&=&\frac{\mb a-\mb a'}{2}\sim\mc{N}(0,\mb I_m/4)+i\mc{N}(0,\mb I_m/4)
\end{eqnarray}
based on the conditioning argument for general decoupling 
\begin{eqnarray}
\mb Q(\bar{\mb a})&=&\expect{\mb Q_{dec}(\bar{\mb a}+\mb\delta,\bar{\mb a}-\mb\delta)}\\
&=&\mb T(\bar{\mb a})+\expect{\mb T(\bar{\mb a})}
-2\sum_{k=1}^m\bar{\mb a}_k^*\mb x\cdot\mb\delta_k^*\mb x\paren{\bar{\mb a}\mb\delta_k^T+\mb\delta_k\bar{\mb a}_k^T}\\
&=&\mb T(\bar{\mb a})-\expect{\mb T(\bar{\mb a})}+\frac12\mb x\mb x^T-\sum_{k=1}^m\bar{\mb a}_k^*\mb x\paren{\bar{\mb a}\mb x^T+\mb x\bar{\mb a}_k^T}\\
&=&\mb T(\bar{\mb a})-\expect{\mb T(\bar{\mb a})}+\frac12\mb x\mb x^T-\frac12\sum_{k=1}^m\paren{\bar{\mb a}\bar{\mb a}_k^*\mb x\mb x^T+\mb x\mb x^Tconj(\bar{\mb a}_k)\bar{\mb a}_k^T}
\end{eqnarray}
Hence the problem boils down to bounding $\Delta_1=\frac1m\sum_{k=1}^m\bar{\mb a}_k\bar{\mb a}_k^*-\frac12\mb I_n$ and $\Delta_2=\frac{1}{m}\sum_{k=1}^m\paren{\mb a_k^*\mb x}^2\mb a_k'\mb a_k'^T$.

\end{proof}



\subsection{Lower bound}
\[\inf_{\mb x,\mb z}\frac{1}{m}\sum_{k=1}^m\abs{\mb a_k^*\mb x}^2\abs{\mb a_k^*\mb z}^2\ge(1-\delta)\paren{\norm{\mb x}2^2\norm{\mb z}2^2+\abs{\mb x^*\mb z}^2}\]
\begin{proof} Let's start by considering real number settings and denote
\[Q(\mb x,\mb z)=\xi\norm{\mb x}2^2\norm{\mb z}2^2-\xi\frac{1}{m}\sum_{k=1}^m\abs{\mb g*\mb x}_k^2\abs{\mb g'*\mb z}_k^2\]

We will consider a localized uniform smoothing $\mu_{\mb x,l}$ on a $l$-height cap around $\mb x$ is defined as
\[\mu_{\mb x,l}(\mb x') =
\begin{cases}
c  & \quad \innerprod{\mb x}{\mb x'}>l\\
0  & \quad \text{others}\\
\end{cases}
\]
where $\mb x,\mb x'\in\bb S^{n-1}$
\[\bb E_{\mb x'\sim\mu_{\mb x,l}}\brac{\mb x'(\mb x')^T}=\alpha_l\mb x\mb x^T+\beta_l\mb I\]
with $\alpha_l\approx l^2$ and $\beta_l\approx\frac1n$, hence
\[\bb E_{\mb x'\sim\mu_{\mb x,l}}\brac{\norm{\mb x'}2^2}=\alpha_l\norm{\mb x}2^2+\beta_l n\quad\bb E_{\mb x'\sim\mu_{\mb x,l}}\brac{\abs{\mb g*\mb x'}_k^2}=\alpha_l\abs{\mb g*\mb x}_k^2+\beta_l\abs{\mb g_k}^2\]


%Gaussian smooth in the space that $\mb z'=\mb z+\mb\delta_{\mb z}$ with $\mb\delta_{\mb z}\sim\mc N(0,\sigma^2\mb I)$, then
%\[\bb E_{\mb\delta_{\mb z}\sim\mc N(0,\sigma^2\mb I)}\brac{\mb z'(\mb z')^T}=\mb z\mb z^T+\sigma^2\mb I\]
%\[\bb E_{\mb\delta_{\mb z}\sim\mc N(0,\sigma^2\mb I)}\brac{\norm{\mb z'}2^2}=\norm{\mb z}2^2+\sigma^2 n\quad\bb E_{\mb\delta_{\mb z}\sim\mc N(0,\sigma^2\mb I)}\brac{\abs{\mb g*\mb z'}_k^2}=\abs{\mb g*\mb z}_k^2+\sigma^2\abs{\mb g_k}^2\]
%




then applying smoothing on the random process $Q$ renders
\begin{eqnarray}
\Gamma_{\mu}Q(\mb x,\mb z)&=&\bb E_{\mb x'\sim\mu_{\mb x,l},\mb z'\sim\mu_{\mb z,l}}\brac{Q(\mb x',\mb z')}\\
&=&\alpha_{lx}\alpha_{lz}Q(\mb x,\mb z)\\
&+&\alpha_{lx}\beta_{lz}\brac{n\norm{\mb x}2^2-\frac1m\sum_k\abs{\mb g*\mb x}_k^2\norm{\mb g'_k}2^2}\\
&+&\beta_{lx}\alpha_{lz}\brac{n\norm{\mb z}2^2-\frac1m\sum_k\norm{\mb g_k}2^2\abs{\mb g'*\mb z}_k^2}\\
&+&\beta_{lx}\beta_{lz}\brac{n^2-\frac1m\sum_k\norm{\mb g_k}2^2\norm{\mb g'_k}2^2}
\end{eqnarray}

By PAC-Bayes method, we know
for any $\mb x,\mb z\in\bb S^{n-1}$,
\[\P\brac{\Gamma_{\mu}Q(\mb x,\mb z)<t+D(\mu\mid\mu_0)}\ge1-e^{-t}\bb E_{\mu_0}\bb E_{\mb g,\mb g'}\brac{e^{Q(\mb x,\mb z)}}\]
Equivalently, with probability larger than $1-e^{-\alpha_{lx}\alpha_{lz}\xi t}\bb E_{\mu_0}\bb E_{\mb g,\mb g'}\brac{e^{\xi Q(\mb x,\mb z)}}$, we have
\begin{eqnarray}
\frac{1}{m}\sum_{k=1}^m\abs{\mb g*\mb x}_k^2\abs{\mb g'*\mb z}_k^2
&\ge&\norm{\mb x}2^2\norm{\mb z}2^2-t-\frac{D(\mu\mid\mu_0)}{\alpha_{lx}\alpha_{lz}\xi}\\
&+&\frac{\beta_{lz}}{\alpha_{lz}}\brac{n\norm{\mb x}2^2-\frac1m\sum_k\abs{\mb g*\mb x}_k^2\norm{\mb g'_k}2^2}\\
&+&\frac{\beta_{lx}}{\alpha_{lx}}\brac{n\norm{\mb z}2^2-\frac1m\sum_k\norm{\mb g_k}2^2\abs{\mb g'*\mb z}_k^2}\\
&+&\frac{\beta_{lx}\beta_{lz}}{\alpha_{lx}\alpha_{lz}}\brac{n^2-\frac1m\sum_k\norm{\mb g_k}2^2\norm{\mb g'_k}2^2}
\end{eqnarray}
Hence, we need some constant an upper bound for $\frac{D(\mu\mid\mu_0)}{\alpha_{lx}\alpha_{lz}\xi}$ and lower bounds for other terms, where
\[\frac{D(\mu\mid\mu_0)}{\alpha_{lx}\alpha_{lz}\xi}=\frac{D(\mu_{\mb x}\mid\mu_{\mb x0})+D(\mu_{\mb z}\mid\mu_{\mb z0})}{\alpha_{lx}\alpha_{lz}\xi}=\frac{n(l_x^2+l_z^2)}{\xi l_x^2l_z^2}\]



\subsubsection{Moment Control}
Let $\lambda_1,\cdots,\lambda_m$ be the eigenvalues of $\sum_{k=1}^m\abs{\mb g'*\mb z}_k^2\mb x_k\mb x_k^T=C^T_{\mb x}~diag(\abs{\mb g'*\mb z}^2)~C_{\mb x}$, note that 
\[\lambda_i\paren{\frac{1}{m}\sum_{k=1}^m\abs{\mb g'*\mb z}_k^2\mb x_k\mb x_k^T}=\sigma^2_i\paren{\frac1{\sqrt{m}}diag(\abs{\mb g'*\mb z})~C_{\mb x}}\]
and for all $\mb z\in\bb S^{n-1}$, with high probability in $\mb g'$
\[\sum_i{\sigma^2_i}=\norm{diag(\abs{\mb g'*\mb z})~C_{\mb x}}{F}^2=\norm{\mb g'*\mb z}2^2\in[1-\eps_1,1+\eps_1]m\]
\begin{eqnarray}
\E_{\mb g}[e^{Q}]&=&e^{\xi\norm{\mb x}2^2\norm{\mb z}2^2}\E_{\tilde{\mb g}}[e^{-\frac{\xi}m\sum_k{\lambda_k}\tilde{g}_k^2}]\\
&\le&e^{\xi\norm{\mb x}2^2\norm{\mb z}2^2}e^{-\frac{\xi}m\sum_k\lambda_k}e^{\frac{\xi^2}{2m^2}\sum_k\lambda^2_k}\\
&\le&e^{\frac{\xi^2}{2m^2}\norm{\mb\lambda}{2m^2}^2}= e^{\frac{\xi^2}{2m^2}\norm{\mb\sigma}4^4}\end{eqnarray}
Then
\[m=n\frac{(l_x^2+l_z^2)}{l_x^4l_z^4}\]
Let 
\[\mu_0(\mb x,\mb z) = c
\begin{cases}
1  & \quad \norm{\mb\sigma}4\le C\log(m)m^{-1/4}\\
e^{-\xi}  & \quad \text{others}\\
\end{cases}
\]
then
\[\E_{\mb g}[e^{Q}]\le e^{\xi^2\log(m)/m}+e^{\xi}e^{-\xi}\]
and
\[\mu\brac{B}\le\mu_{\mb x}\brac{\norm{\mb x}4\ge C_1m^{-1/4}}+\mu_{\mb z}\brac{\norm{\mb g'*\mb z}{\infty}>C_2\log(m)}\]
in this case, the original KL divergence need to be modified with a small increment $\mu\brac{B}/{\alpha_{lx}\alpha_{lz}}$.


For simplicity, we are going to consider a truncated version of the original function
\[\hat{Q}(\mb x,\mb z)=\norm{\mb x}2^2\norm{\mb z}2^2-\frac{1}{m}\sum_{k=1}^m\abs{\mb g*\mb x}_k^2\abs{\widehat{\mb g'*\mb z}}_k^2\ge Q(\mb x,\mb z)\]
let $\lambda_1,\cdots,\lambda_m$ be the eigenvalue of $\frac{1}{m}\sum_{k=1}^m\abs{\widehat{\mb g'*\mb z}}_k^2\mb x\mb x^T$
then
\begin{eqnarray}
\E_{\mb g}[e^{Q'}]&=&e^{\xi\norm{\mb x}2^2\norm{\mb z}2^2}\E_{\tilde{\mb g}}[e^{-\xi\sum_k{\lambda_k}\tilde{g}_k^2}]\\
&\le&e^{\xi\norm{\mb x}2^2\norm{\mb z}2^2}e^{-\xi\sum_k\lambda_k}e^{\frac{\xi^2}2\sum_k\lambda^2_k}\\
&\le&e^{\frac{\xi^2}2\norm{\mb\lambda}2^2}
\end{eqnarray}
Then we are going to consider two sets for $\mb\lambda$
\begin{itemize}
\item With some "good" choice of $\mb x$ and $\mb z$, we have $\norm{\mb \lambda}2^2\le\frac{pl(n)}{n}$
\item Otherwise, $\norm{\mb \lambda}2^2>\frac{pl(n)}{n}$, and is contained in $\sum_{i=i^*}^m \lambda_i^2>\frac{pl(n)}{n}$. Here, we introduced the truncation to deal with the heavy tail of $\norm{\hat{\mb z}}4$.
\end{itemize}

\end{proof}

\subsubsection{Oversampled Fourier transform of a short vector}
In this problem, the oversampled Fourier transform of a short vector carries a lot of interests, this part is devoted to have a detailed discussion for its performance.
Let $\mb z\in\bb S^{n-1}$, and its oversamples Fourier transform $\hat{\mb z}$. One trivial bound through Parseval's theorem and general vector norm property is 
\[\norm{\hat{\mb z}}2=n^{\frac12}\norm{\mb z}2,\quad n^{\frac14}\norm{\mb z}2\le\norm{\hat{\mb z}}4\le n^{\frac12}\norm{\mb z}2\]
Because of the local smoothness of an oversampling Fourier matrix,  we are going to apply a segmentation of the support set $\Omega=\set{1,\cdots,m}=\bigcap_{j=1}^{m/n}\Omega_j$. For simplicity, we will assume $n=2^k$ and $\frac{m}{n}=p$ for some positive integers $k$, $p$, then each subset can be defined as
\[\Omega_j=\set{j,j+p,\cdots,j+(n-1)p}\]
Th main advantage offered by this segmentation is that now any $\hat{\mb z}_{\Omega_j}$ is a unitary transformation of the $\mb z$, which preserves independence and variance.
\begin{eqnarray}
\P\set{\sum_{i=i^*}^n\abs{\hat{\mb z}}_{(i)}^4\ge\beta}
&\le&\P\set{\exists~j\quad\text{s.t.}\sum_{i=i_j^*}^m\abs{\hat{\mb z}_{\Omega_j}}_{(i)}^4\ge\beta/p}\\
&\le&p\P\set{\sum_{i=i_1^*}^m\abs{\hat{\mb z}_{\Omega_1}}_{(i)}^4\ge\beta/p}
\end{eqnarray}
where $i^*$ and $i_j^*$ are the largest integers chosen such that 
\[\sum_{i=1}^{i^*-1}\abs{\hat{\mb z}}_{(i)}^2\le\alpha,\quad\sum_{i=1}^{i_j^*-1}\abs{\hat{\mb z}_{\Omega_j}}_{(i)}^2\le\alpha/p\]
Renyi's representation asserts that the order statistics of a sample of independent exponentially distributed random variables are distributed as partials sums of independent exponentially distributed random variables. Let $x_{(1)}\ge x_{(2)}\ge\cdots\ge x_{(n)}$ be the ordered exponential random variables with parameter $1$, then
\[x_{(k)}=_d\frac{x'_k}{k}+\cdots+\frac{x'_z}{n}\]
hence
\[\E[x_{(k)}]=\sum_{i=k}^n\frac1i,\quad var(x_{(k)})=\sum_{i=k}^n\frac1{i^2}\]

The minimum $x_{(n)}$ is exponential with parameter $n$. Conditioned on $x_{(n)}$, the second smallest value $x_{(n-1)}$ is distributed like the sum of $x_{(n)}$ and an independent exponential random variable with parameter $n-1$.

\begin{itemize}
\item $i_j^*>i_0=\frac{n}{pl(n)}$
\item $\abs{\mb q}_{(j_0)}<pl(n)\implies\le\norm{\check{\mb q}}4^4$
\item $\norm{\check{\mb q}}4^4<\frac{\beta}{p}$
\end{itemize}







